Mutual Mobile Membranes with Timers

A feature of current membrane systems is the fact that objects and membranes are persistent. However, this is not true in the real world. In fact, cells and intracellular proteins have a well-defined lifetime. Inspired from these biological facts, we define a model of systems of mobile membranes in which each membrane and each object has a timer representing their lifetime. We show that systems of mutual mobile membranes with and without timers have the same computational power. An encoding of timed safe mobile ambients into systems of mutual mobile membranes with timers offers a relationship between two formalisms used in describing biological systems.

==> eptcsdata.tex <==
\providecommand{\event}{R.J.Back, I.Petre, E. de Vink (Eds.): Computational\\
Models for Cell Processes (CompMod 2009)}
\providecommand{\volume}{6}
\providecommand{\anno}{2009}
\providecommand{\firstpage}{1}
\providecommand{\eid}{1}

